SoK: Oracles from the Ground Truth to Market Manipulation

One fundamental limitation of blockchain-based smart contracts is that they execute in a closed environment. Thus, they only have access to data and functionality that is already on the blockchain, or is fed into the blockchain. Any interactions with the real world need to be mediated by a bridge service, which is called an oracle. As decentralized applications mature, oracles are playing an increasingly prominent role. With their evolution comes more attacks, necessitating greater attention to their trust model. In this systemization of knowledge paper (SoK), we dissect the design alternatives for oracles, showcase attacks, and discuss attack mitigation strategies.

==> sections/table_aggregation.tex <==
% !TEX root = ../main.tex

\begin{table*}[ht!]

    \renewcommand{\arraystretch}{1.3}
    
    \centering
    
    \begin{tabular*}{0.9\textwidth}{@{\extracolsep{\fill}} llccccccccccccc}
    
    \textit{Category} &
    \textit{Example} & 
    \headrow{No single trusted party} & %
    \headrow{Low latency} &  %
    \headrow{Availability} &
    \headrow{Data Integrity} & % data quality
    \headrow{Outlier Detection} &
    \headrow{Handle Stale Data} & %
    \headrow{Cost Effective} &
    \headrow{ } & % Something about format decay
    \headrow{ } \\ \hline 
    
    Single source (no aggregation)    & 	&	&	&\full	&	&\full	&\full	&\full	&&\\
    Flat (mean, median, etc)    &	&	&\prt	&\full	&\prt	&\full	&	&\full		&&\\
    Weighted (time, volume)	&				&\prt	&\full	&\full	&	&	&\full		&\full	&&\\ 
    Random Selection    &  		&\prt	&\full	&\full	&	&\full	&\full	&\full		&&\\ 
    % COLUMN    & 		&	&\full	&\full	&\prt	&	&	&\full	&\full	&\full	&\full	&&\\ 
    \\
                                                                                        
    \end{tabular*}
    
    \caption{CAPTION. \full~ indicates the category of client is awarded the benefit in the corresponding column. \prt~partially awards the benefit. Details provided inline.}
    \label{tab:prims}
    \end{table*}
      
    
    
    
    
    
    
    
    
    
    
    
    
    
    

==> sections/table_dispute.tex <==
% !TEX root = ../main.tex


% Dispute:
% 	- Rows: 
% 		Preventive: Staking (collateral or reputation),   
% 		Corrective: Reversion, (Reconciliation), Recursive
% 	- Columns: Reliance of single trusted party, low latency (finality in 2 mins? ), availability, data quality (Accuracy), cost effective, influenced by external economics (economical exogenous)


\begin{table*}[ht!]

    \renewcommand{\arraystretch}{1.3}
    
    \centering
    
    \begin{tabular*}{0.9\textwidth}{@{\extracolsep{\fill}} llccccccccccccc}
    
    \textit{Category} &
    \textit{Example} & 
    \headrow{No single trusted party} & %
    \headrow{Low latency} &  %
    \headrow{Availability} &
    \headrow{Data Accuracy} & % Data quality
    \headrow{Economical Exogenous} &
    \headrow{ROW} & %
    \headrow{ } & % Something about format decay
    \headrow{ } \\ \hline 
    
    \textbf{Preventive:}    & 	&	&	&\full	&	&\full	&\full	&&\\
    Staking (collateral or reputation)    &	&	&\prt	&\full	&\prt	&\full	&		&&\\
    \textbf{Corrective:}	&				&\prt	&\full	&\full	&	&	&\full		&&\\ 
    Reversion    &  		&\prt	&\full	&\full	&	&\full	&\full		&&\\ % data quality
    (Reconciliation)    & 		&	&\full	&\full	&\prt	&	&		&&\\ 
    Recursive    & 			&	&	&	&	&	&\full		&&\\ 
    % Column 8	&				&\prt	&\full	&	&	&	&\full	&&\\
    \\
                                                                                        
    \end{tabular*}
    
    \caption{CAPTION. \full~ indicates the category of client is awarded the benefit in the corresponding column. \prt~partially awards the benefit. Details provided inline.}
    \label{tab:prims}
    \end{table*}
      
    
    
    
    
    
    
    
    
    
    
    
    
    
    
